Scalable Graph Convolutional Network Training on Distributed-Memory Systems

Graph Convolutional Networks (GCNs) are extensively utilized for deep learning on graphs. The large data sizes of graphs and their vertex features make scalable training algorithms and distributed memory systems necessary. Since the convolution operation on graphs induces irregular memory access patterns, designing a memory- and communication-efficient parallel algorithm for GCN training poses unique challenges. We propose a highly parallel training algorithm that scales to large processor counts. In our solution, the large adjacency and vertex-feature matrices are partitioned among processors. We exploit the vertex-partitioning of the graph to use non-blocking point-to-point communication operations between processors for better scalability. To further minimize the parallelization overheads, we introduce a sparse matrix partitioning scheme based on a hypergraph partitioning model for full-batch training. We also propose a novel stochastic hypergraph model to encode the expected communication volume in mini-batch training. We show the merits of the hypergraph model, previously unexplored for GCN training, over the standard graph partitioning model which does not accurately encode the communication costs. Experiments performed on real-world graph datasets demonstrate that the proposed algorithms achieve considerable speedups over alternative solutions. The optimizations achieved on communication costs become even more pronounced at high scalability with many processors. The performance benefits are preserved in deeper GCNs having more layers as well as on billion-scale graphs.

==> OLD-response.tex <==
\centerline{\Huge \textbf{Revision Cover Letter}}
\medskip

\noindent
We thank the reviewers for their careful analysis and suggested improvements. Below, we elaborate on our significant revisions and experiments performed to address all the concerns and strengthen our work and submission. 


\section*{Meta-review}

\revComment{MR}{The reviewers generally found the work solid and interesting, but they also identified several opportunities for improvement. We encourage you to revise your paper taking into consideration all of the reviewer comments, and submit an improved version of the manuscript.
Major Revision Items:
\begin{enumerate}
    \item Justify relevance of your work to VLDB better. (R1.W1)
    \item Add experiments on CPU vs. GPU comparison. (R1.W2)
    \item Clarify contributions in terms of sparse matrix usage. (R1.W3)
    \item State the main contribution more clearly. (R3.W1)
    \item Add missing related work. (R3.W2)
    \item Revise the mathematical statement in Section 3.1. (R3.W3)
    \item Clarify if the proposed method can be used with other types of GNNs. (R4.W1/D1)
    \item Evaluate scalability on larger graphs. (R4.W3/D2)
    \item Clarify the task used in the experimental evaluation as well as showing if the GCN predictive performance degrades due to optimizations or not. (R4.D3)
    \item Add an ablation study to analyze the relative impacts of hypergraph partitioning model and randomized hypergraph model. (R4.D4)
\end{enumerate}
}

\revResponse{We are grateful for this summary of the required revisions. We have carefully revised our paper and addressed each of these points successfully. 
\begin{enumerate}
    \item We have added content that significantly strengthens the justification of our work in the context of VLDB. Overall, we have extended our discussions about related research in our community, e.g., highlighting many VLDB papers on scalable machine learning training,  parallel/distributed GNNs, graph partitioning and communication schemes, and promising VLDB research based ideas for ongoing and future work. 
    \item We have added new experiments for CPU versus GPU comparison, which further show how our solution and communication scheme have significant advantages, and how the CPU based approach achieves the best scalability in the experiments.
    \item We have reorganized the related work and clarified how we devise a hypergraph model that exploits the sparsity of the adjacency matrix, to better distinguish our additional contributions in this direction.
    \item In the introduction we have further highlighted our contributions and novelties.
    \item We have added the new references.
    \item We have made this correction.
    \item Our solution is indeed applicable to other types of GNNs and we have added a section to discuss this. We implemented a GAT version of our solution as an example, and released our GAT implementation in our public codebase.
    \item We have evaluated our models on the recommended billion-scale \texttt{ogbn-Papers100M} dataset, which confirms scalability on larger graphs.
    \item We clarify that the task considered is node classification, and there is no change in prediction performance. We have added an evaluation of predictive performance which shows that the model accuracy is maintained for any number of processors.
    \item The new ablation study, figure, and analysis now help to directly compare our randomized/stochastic (SHP) model against the HP model, showing the relative benefits of SHP in terms of both running time and communication volume.
\end{enumerate}
}

\section*{Reviewer 1}

\revComment{R1.S}{1. The proposed approach achieves scalability by replacing the blocking broadcast communications in existing approaches with non-blocking point-to-point communications.\\
2. The paper took into consideration the randomness of communication operations performed in mini-batch training. And the paper proposed a randomized hypergraph partitioning model for sampling training strategy.}

\revResponse{Thank you. These are indeed important contributions of our work. We have now additionally shown how our point-to-point communication scheme benefits the CPU performance also when compared with the GPU approaches. We now also better showcase the performance of the randomized/stochastic (SHP) model as advised.}


\revComment{R1.O1/W2}{The paper focused on GCN training on large-scale CPU clusters which is suitable for sparse problems. It could be better to conduct experiments on comparing the proposed CPU based method with GPU based method to show the superiority of the proposed method.}

\revResponse{
%As indeed pointed out by the reviewer, GPU clusters are not well-suited for algorithms that are focused on optimizing communication operations, and where the sparsity of the problem is important to exploit. 
To address this comment, we implemented and evaluated a new GPU version of our distributed algorithm by using PyTorch with NCCL backend.
We present new strong scaling results in Figure 3, where we use a cluster of 30 GPUs to test the GPU version of our algorithm~(i.e., HP, GP, RP) against the original GPU version of CAGNET.
We also use these findings to compare and motivate the significant improvements we can achieve on CPU clusters. 
%Our solutions, HP and GP, perform better than CAGNET even on a small number of GPU as compared to large-scale CPU cluster experiments.
The HP model performance on the CPU cluster is better than that on the GPU cluster in many settings, which we highlight for \texttt{amazon0601} and \texttt{roadNet-CA} datasets.
We discuss the reasons for this under ``Parallel Running Times'' in Section~5. In brief, the NCCL backend involves high communication overheads that eclipse the effects of parallelizing computations, and the 
%This is because the NCCL backend cannot provide the necessary efficiency for speedup on GPUs, where the proportion of total running time that is spent on local computation is small.
%Therefore the parallelization gains do not amortize the time spent for communication.
communication volume optimizations are also not as effective as with MPI. 
%, and suffers higher latency costs.
While no suitable larger GPU clusters were available for our experiments, we expect that the performance improvement of HP over alternatives is expected to be more pronounced at much larger GPU counts, similar to the trend seen in the CPU cluster results.
Our optimizations are very successful for sparse problems with high scalability to many processors especially where there are network limitations, and our solution has applicability to both full-batch and mini-batch training.
}

\revComment{R1.O2}{Only two baselines (DGL and CAGNET) were compared in experiments, which is too short. Other distributed GNN training methods and systems, could be compared with, are omitted, such as: PaGraph, DGCL, Dorylus.}

\revResponse{We have now enhanced the paper to discuss a broader range of systems, and added a new subsection on ``Comparison against SOTA'' in Section~5, where we compare the running time of our GPU implementation (HP) against popular distributed GPU systems. Since our optimizations are proposed for large-scale CPU clusters, we expect that GPU-targeted optimizations would further improve our performance. Since our primary task is to optimize communication operations in parallel full-batch and mini-batch training of GCNs, DGL and CAGNET are widely utilized as state-of-the-art solutions and are the natural baselines to our work.
To achieve higher scalability and avoid bottlenecks, we develop a fully distributed approach without need for graph data replication, and avoiding parameter server approaches where several worker processes synchronously or asynchronously update parameters stored in a server.

We also note that the listed references diverge from our work and other baselines as follows. 
PaGraph is built on DGL and it is only able to run on single node with several GPUs whereas the tested algorithms in our experiments are able to run on multiple nodes in a fully distributed environment. 
%We note that PaGraph is using DGL itself.
PaGraph has orthogonal aims as it accelerates sampling-based training. % to improve data loading and sampling time. 
%The L-hop neighborhood is replicated across partitions mainly to improve the sampling process. 
%Most importantly, this algorithm is 
DGCL is a communication planning library, and not publicly available. Its goal is to avoid network contention.
Both systems study replication/caching with data-parallelism, which can be a new orthogonal direction of research beyond our graph and hypergraph partitioning based approaches.
%to avoid communication on slower links. Considering vertex replication in both graph and hypergraph partitioning is an orthogonal new direction of research.
%Hence, comparison against this library is not fair for any algorithms. 
%We thank the reviewer for pointing out this reference which we consider as a new potential research direction.  
Dorylus uses AWS cloud serverless computing services and performs asynchronous parameter updates on a server. % using an update mechanism that achieves convergence guarantees.
Hence, Dorylus largely diverges from our work since our solution performs synchronous updates to parameters. % and does not affect predictive and convergence properties of GCN training.
}

\revComment{R1.O3}{In section 5, it is confused that does ‘RP’ refer to simple random partitioning algorithm or randomized hypergraph partitioning algorithm? It could be better to clarify that.}

\revResponse{We appreciate this suggestion and now better clarify the distinction by using the term ``stochastic hypergraph partitioning'' (SHP). In Section~5 we now use HP, GP, RP, and SHP to denote the various methods.}

\revComment{R1.O4}{It could be better to evaluate the proposed randomized hypergraph partitioning algorithm performance in Table 2, Figure 4, 5, instead of just in communication volume evaluation(Figure 7).}

\revResponse{We now include an updated Figure~5 where we report run time as well as communication volume comparisons. This helps us to more clearly evaluate the performance benefits of SHP (randomized/stochastic hypergraph partitioning) over HP under ``Stochastic Hypergraph Model'' in Section~5, as suggested.
SHP performs worse than HP in full-batch training since it partitions a completely different hypergraph model (a merged hypergraph generated from sampling many subgraphs). 
However, SHP encodes the sampling randomness and becomes better than HP when mini-batch training is applied. Therefore, we consider Table~2 to be already complex and for ease of exposition, we present SHP in a separate context as described above.
}

\revComment{R1.W1}{This paper accelerates GNN Training and is not very relevant to VLDB. Justify the relevancy to VLDB.}

\revResponse{
We have now extended our related work discussions on closely related research in the context of VLDB, e.g., parallel/distributed GNNs, scalable training, 
large-scale graph partitioning, and communication schemes in this context. Methods for graph partitioning that tackle scalability in network bound applications~\cite{ching2015one}, study communication overheads~\cite{gill2018study}, adaptively determine partitioning strategies at run time~\cite{fan2021graphscope}, or are application-driven~\cite{fan2022application}, have  generated great interest in recent VLDB conferences. These motivate the need for our solution that employs GNN-specific considerations during the partitioning stage.

The research areas we tackle have been widely considered in the VLDB community, including parallel and distributed processing for graph analytics~\cite{lu2014large,han2014experimental,sarwat2013horton+,tian2013think,yan2014blogel,zhao2013partition} and GNNs~\cite{liu2020g3, parallel2021,min2021large,zhang2020agl,zhang2021Cerebro,zheng2022bytegnn,zhou2021accelerating,tgl2022,peng2022sancus,miao2021het}.
%to reducing communication and caching towards improving GNN model efficiency~\cite{peng2022sancus,miao2021het}.
%In particular, two recent papers that received VLDB best paper awards have dealt with related problem domains of avoiding broadcast communication in data-parallel GNNs~\cite{peng2022sancus} and caching for GNN model efficiency~\cite{miao2021het}.
%Sancus~\cite{peng2022sancus} adaptively avoids broadcast communications to reduce network traffic in data-parallel GNNs.
%HET~\cite{miao2021het} improves the efficiency of huge GNN embedding models via caching methods.
We have revised our paper to further highlight the relationship to these studies within the VLDB community. 
In the conclusions, we have now also included several directions for future work that are of interest to our community.}


\revComment{R1.W3}{What is the contribution on Sparse Matrix?}

\revResponse{Our work makes several significant contributions including a scalable GNN system that exploits sparse matrix patterns in the training process; we have now highlighted them better in the paper, mainly in the introduction and Section~2.3 on ``Data-Parallelization for GNNs''. Our approach exploits the sparse matrix connectivity patterns for effective partitioning to then employ distributed parallel SpMM for convolution with DMM for feature propagation. The captured sparsity patterns benefit our communication scheme optimized for GCN training by reducing overall communication volume based on a hypergraph model of the original graph. Our data partitioning scheme thereby simultaneously considers the requirements of forward propagation as well as backpropagation during the training phase (aggregating features/gradients, and updating parameter matrices). We discuss the connection to sparse matrix techniques in a new subsection under related work (Section~2.3).}


\thispagestyle{plain}


\section*{Reviewer 3}

\revComment{R3.S}{1. Solid technical contributions.\\
2. Well written and easy to read.\\
3. Experiments are well done and supports the claim.}

\revResponse{We thank the reviewer for these positive comments.}


\revComment{R3.W1}{In introduction, there are a few times with "graph and hypergraph partitioning models", "hypergraph and graph partitioning", which is a bit confusing about which is your contribution. Can we simply say "we developed hypergraph partitioning model to reduce communications, which outperforms existing graph partitioning models"?}

\revResponse{Thank you, the suggested edits improve clarity and we have updated sentences in our introduction accordingly.}

\revComment{R3.W2}{There are works on doing matrix multiplication in cloud data processing systems. Not sure where the literature is as of now, but here are two early works: Cumulon, SystemML. Please add some related work discussions.}

\revResponse{Thank you for the interesting references. We have added discussions of such systems in the related work. Cloud-based adaptations can indeed offer interesting directions for future work.}

\revComment{R3.W3}{Section 3.1, "a feature matrix $H^k\in R^{n\times d_k}$, should it be $H^0$ and $d_0$ instead so that it is picked up in the feed forward equations when $k = 1$?}

\revResponse{We are grateful for this keen observation. The feature matrix $H^0$ is indeed required as input, and we have added a detail in Section~3.1 to clarify that the computations begin with $H^0$ before being fed through layers $k=1,\ldots,L$.}


\thispagestyle{plain}


\section*{Reviewer 4}

\revComment{R4.S}{1. Scalable GCN training is a natural and important problem to study.\\
2. The idea of using hypergraph model to encode the expected communication volume is interesting.\\
3. Related works are well presented, and the techniques are explained with examples.}

\revResponse{We thank the reviewer for the positive feedback, and appreciate the interest in the problem we are solving. We have now further highlighted the novelties as requested, as well as introduced some additional findings during this revision period.}

\revComment{R4.D1/W1}{The proposed method only works for GCN rather than general GNNs. Although most GNNs follow the message-passing paradigm (i.e., consecutive SpMM followed by DMM operations) used in GCN, some GCN variants are more complex, such as GAT [1]. Besides, some methods decouple this paradigm and finish the SpMM or DMM operations in advance, such as SGC [2] and APPNP [3]. It would be better to see if the proposed method can adapt to various GNNs, such as APPNP, SGC, and GAT.}

\revResponse{As correctly pointed out, general GNN models mainly differ from GCNs only in the way messages are created and combined between vertices.
We have added a new Section~4.3.4 named 
''Extension to GNNs'' in the revised paper.
Here, we elaborate why modifications in the order of SpMM and DMM, or inclusion of additional intermediate mathematical operations, do not affect the message communication patterns between vertices and therefore our communication scheme remains valid.
Thus our partitioning method can directly be applied for such cases. Some additional operations may need to be included alongside the SpMM/DMM calculations to design other GNNs.
We also provide new sample code, in our public GitHub repository, that implements a GAT model by utilizing our partitioning methods and communication scheme.
}

\revComment{R4.W2}{The novelty of the work needs to be justified more.}

\revResponse{To address this comment, we now better clarify our novelties, mainly in the abstract and introduction.
To summarize, our approach significantly improves scalability while maintaining model predictive performance, by designing non-blocking point-to-point communications for GNN workloads, and exploits the sparsity in connectivity patterns in GNN training when deciding the partitioning such that these point-to-point communications result in low message volume.
We also introduce a novel randomized/stochastic hypergraph partitioning (SHP) model to account for the randomness of communication operations during mini-batch training. 
During this revision period we have further introduced new content and useful findings in the paper: i) the quantified benefits of our communication scheme, and greater scalability achieved on CPU clusters, ii) the generalizability of our solution to others types of GNNs and the minor modifications required to support different combinations of SpMM/DMM, iii) the scalability to billion-scale graphs.}

\revComment{R4.D2/W3}{Scalability analysis on large graphs is preferred. The largest graph tested is cit-Patents, which only consists of 3.7 million nodes. I wonder how the proposed solution performs on billion-scale graphs (such as Papers100M: https://ogb.stanford.edu/docs/nodeprop/\#ogbn-papers100M).}

\revResponse{
To address this comment, we have added a new subsection named 
''Scalability to Billion-scale Datasets'' in Section~5 of the revised paper.
Here, we include new experiments to test scalability to the billion-scale dataset \texttt{ogbn-Papers100M}. We find that the reduction in communication volume enjoyed by our HP model allows for much better scalability when compared with RP.}

\revComment{R4.D3}{It is unclear what task is used for the experimental evaluation. Besides, it is unclear whether the optimizations in this paper will harm the predictive performance of GCN.}

\revResponse{We are grateful for this suggestion and have clarified these points in the revision.
The task evaluated is node classification, and there is no change in prediction performance.
We perform new experiments and confirm that parallelizing our system to more processors does not have any negative impact on the predictive performance.
In our scalability experiments, when comparing different partitioning models, we ran the parallel GCN algorithm for node classification with random vertex features and random label data for five epochs, and used negative log likelihood loss. These datasets did not have any class labels provided.
To address this comment, we modified subsection named ''Communication Costs.'' in Section~6 ``Experimental Results'' to better clarify our experimental settings.
We have also added a new subsection named ''Predictive Performance.'' with a new Figure~4c in Section~5 ''Experimental Results'' of the revised paper.
In this new section, we compared the accuracy performance of HP on different numbers of GPUs against serial DGL implementation of GCN. Here, we use the \texttt{Cora} dataset that has training and test labels available, and find that the accuracy of the model is maintained on increasing the processor count.
}

\revComment{R4.D4}{It is better to add an ablation study to measure the individual influence of the hypergraph partitioning model and the randomized hypergraph model in mini-batch training.}

\revResponse{To address this comment, we add new ablation studies to compare the parallel running time performance and communication cost metrics during mini-batch training, comparing SHP against the natural baseline HP model.
We implemented mini-batch training method in our new GPU implementation of parallel GCN and also included the new codes in our GitHub repository.
While the randomized/stochastic partitioning method (SHP) repeatedly samples subgraphs as mini-batches, thereby accounting for randomness in communications, the HP approach partitions the hypergraph model from the original graph and does not encode this randomness, thus incurring higher message volume and overall running time.
In this regard, we have modified the subsection named ''Stochastic Hypergraph Model.'' and Figure~5 in Section~5 ''Experimental Results'' in the revised paper.}

\revComment{R4.D5}{Minor Comments: Abstract: achieves -> achieve; Introduction, Page 1: Graph Neural Networks -> Graph Convolutional Networks.}

\revResponse{Thank you, we have addressed these in the revised paper.}


==> plot1.tex <==
\begin{tikzpicture}
\begin{loglogaxis}[xtick={ 16, 32,64,128,256,512},xticklabels={ 16, 32,64,128,256,512}, ytick={0.25,0.5,1,2,4,8,16}, yticklabels={0.25,0.5,1,2,4,8,16}, grid=major,xlabel= Processors, ylabel=Time,scale=0.7]
\addplot[very thick, line width=1.3pt, mark=x,color=red,mark options={scale=2.5}] coordinates {
(16,2.9439112499999998)
(32,2.08425175)
(64,1.8044660000000001)
(128,1.2968977499999998)
(256,0.82226)
(512,0.64591125)
};  

\addplot[very thick, line width=1.3pt, mark=x,color=blue,mark options={scale=2.5}] coordinates {
(16,3.87004725)
(32,3.040419)
(64,2.74584275)
(128,2.14514325)
(256,1.7165154999999999)
(512,1.14641525)
};  

\addplot[very thick, line width=1.3pt, mark=x,color=green,mark options={scale=2.5}] coordinates {
(16,9.61429575)
(32,8.72558575)
(64,7.503812250000001)
(128,6.62002075)
(256,5.13485975)
(512,3.9295947500000002)
};  

\legend{H-GCN,G-GCN,GCN}
\end{loglogaxis}
\end{tikzpicture}












==> plot2.tex <==
\begin{tikzpicture}
\begin{loglogaxis}[xtick={ 16, 32,64,128,256,512},xticklabels={ 16, 32,64,128,256,512}, ytick={0.125,0.25,0.5,1,2,4}, yticklabels={0.125,0.25,0.5,1,2,4}, grid=major,xlabel= Processors,ylabel=Time, scale=0.7]
\addplot[very thick, line width=1.3pt, mark=x,color=red,mark options={scale=2.5}] coordinates {
(16,2.9439112499999998)
(32,2.08425175)
(64,1.8044660000000001)
(128,1.2968977499999998)
(256,0.82226)
(512,0.64591125)
};  

\addplot[very thick, line width=1.3pt, mark=x,color=blue,mark options={scale=2.5}] coordinates {
(16,3.14388475)
(32,2.7255527500000003)
(64,2.3144324999999997)
(128,1.82869225)
(256,1.3395497500000002)
(512,1.2973180000000002)
};  

\addplot[very thick, line width=1.3pt, mark=x,color=green,mark options={scale=2.5}] coordinates {
(16,3.3812135000000003)
(32,2.443737)
(64,2.25420725)
(128,1.86016175)
(256,1.53325925)
(512,1.24968225)
};  

\legend{t1x,t2x,t4x}
\end{loglogaxis}
\end{tikzpicture}



==> plot3.tex <==
\begin{tikzpicture}
\begin{axis}[grid=major,width=7cm,height=6.5cm,
		xlabel=Layers,
		ylabel=Speedup,
		cycle list name=color,scale=0.8]
	\addplot coordinates {
		(2,6.66504984078364)
		(3,6.24687274913336)
		(4,5.49689934335515)
		(5,5.08007580827562)
		(6,5.01561670743084)
		(7,4.63643908852094)
		(8,4.63192987972143)
	};
	\addlegendentry{f100-t1x}
	
	\addplot coordinates {
		(2,12.1564316877378)
		(3,9.65487490840108)
		(4,8.15741897628118)
		(5,7.68465283693396)
		(6,7.13330245834621)
		(7,6.86111990068674)
		(8,6.61836196837654)
	};
	\addlegendentry{f50-t1x} 
	
\end{axis}

\end{tikzpicture}






















%(2,)
%(3,)
%(4,)
%(5,)
%(6,)
%(7,)
%(8,)






==> table1_old.tex <==
\begin{table*}[t]
\renewcommand{\arraystretch}{0.9}
\caption{Performance comparison of H-GCN, G-GCN and R-GCN} 
\label{tables:table1}
\centering
\setlength\tabcolsep{5pt}
\begin{tabular}{l*5r||*6r}
& \multicolumn{5}{c}{256} & \multicolumn{6}{c}{512} \\
\cmidrule(r){2-6}\cmidrule(r){7-12}
& & \multicolumn{2}{c}{Volume} & \multicolumn{2}{c}{Messages} & & \multicolumn{2}{c}{Volume} & \multicolumn{2}{c}{Messages} & \\
\cmidrule(r){3-4}\cmidrule(r){5-6}\cmidrule(r){8-9}\cmidrule(r){10-11}
& \multicolumn{1}{c}{R}   & \multicolumn{1}{c}{Avg} & \multicolumn{1}{c}{Max}         & \multicolumn{1}{c}{Avg} & \multicolumn{1}{c}{Max} & \multicolumn{1}{c}{R}   & \multicolumn{1}{c}{Avg} & \multicolumn{1}{c}{Max}         & \multicolumn{1}{c}{Avg} & \multicolumn{1}{c}{Max} & \multicolumn{1}{c}{S} \\
\cmidrule(r){2-6}\cmidrule(r){7-12}
\multirow{3}{*}{cit-Patents}      & 0.55 & 0.14 & 0.24 & 0.93 & 1.00 & 0.56 & 0.17 & 0.28 & 0.67 & 0.87 & 3.90  \\
                                  & 0.55 & 0.16 & 0.32 & 0.95 & 1.00 & 0.49 & 0.19 & 0.51 & 0.75 & 0.95 & 3.08  \\
                                  & 0.99 & 0.90 & 0.75 & 0.98 & 1.00 & 1.15 & 0.87 & 0.56 & 0.89 & 0.92 &       \\
\cmidrule(r){2-12}\multirow{3}{*}{coPapersDBLP}     & 0.21 & 0.06 & 0.10 & 0.70 & 0.92 & 0.19 & 0.06 & 0.10 & 0.39 & 0.68 & 5.37  \\
                                  & 0.44 & 0.07 & 0.17 & 0.91 & 0.98 & 0.39 & 0.06 & 0.20 & 0.54 & 0.75 & 3.26  \\
                                  & 0.48 & 0.91 & 0.60 & 0.77 & 0.94 & 0.49 & 1.08 & 0.48 & 0.73 & 0.90 &       \\
\cmidrule(r){2-12}\multirow{3}{*}{com-Amazon}       & 0.25 & 0.07 & 0.17 & 0.29 & 0.52 & 0.33 & 0.08 & 0.19 & 0.13 & 0.28 & 5.99  \\
                                  & 0.29 & 0.08 & 0.16 & 0.38 & 0.62 & 0.34 & 0.09 & 0.20 & 0.17 & 0.38 & 5.49  \\
                                  & 0.88 & 0.91 & 1.08 & 0.76 & 0.84 & 1.00 & 0.88 & 0.95 & 0.77 & 0.73 &       \\
\cmidrule(r){2-12}\multirow{3}{*}{com-Youtube}      & 0.56 & 0.30 & 0.46 & 0.91 & 1.00 & 0.60 & 0.36 & 0.59 & 0.71 & 0.98 & 4.08  \\
                                  & 0.98 & 0.33 & 1.56 & 0.99 & 1.00 & 0.93 & 0.30 & 1.67 & 0.87 & 1.00 & 2.42  \\
                                  & 0.58 & 0.91 & 0.29 & 0.92 & 1.00 & 0.65 & 1.19 & 0.35 & 0.82 & 0.98 &       \\
\cmidrule(r){2-12}\multirow{3}{*}{flickr}           & 0.75 & 0.35 & 0.56 & 0.87 & 1.00 & 1.23 & 0.37 & 0.53 & 0.74 & 1.00 & 4.60  \\
                                  & 4.88 & 0.26 & 2.12 & 1.00 & 1.00 & 6.55 & 0.34 & 3.42 & 0.92 & 1.00 & 0.84  \\
                                  & 0.15 & 1.34 & 0.26 & 0.88 & 1.00 & 0.19 & 1.08 & 0.16 & 0.80 & 1.00 &       \\
\cmidrule(r){2-12}\multirow{3}{*}{roadNet-CA}       & 0.10 & 0.01 & 0.01 & 0.02 & 0.04 & 0.07 & 0.01 & 0.01 & 0.01 & 0.03 & 11.07 \\
                                  & 0.09 & 0.01 & 0.01 & 0.02 & 0.05 & 0.06 & 0.01 & 0.01 & 0.01 & 0.03 & 9.73  \\
                                  & 1.13 & 0.74 & 0.69 & 1.00 & 0.83 & 1.13 & 0.81 & 0.75 & 1.00 & 1.00 &       \\
\cmidrule(r){2-12}\multirow{3}{*}{road\_central}    & 0.11 & 0.01 & 0.01 & 0.02 & 0.05 & 0.09 & 0.01 & 0.01 & 0.01 & 0.03 & 8.46  \\
                                  & 0.09 & 0.01 & 0.01 & 0.02 & 0.05 & 0.09 & 0.01 & 0.01 & 0.01 & 0.02 & 7.96  \\
                                  & 1.13 & 0.78 & 0.69 & 1.10 & 1.00 & 1.00 & 0.79 & 0.81 & 1.10 & 1.08 &       \\
\cmidrule(r){2-12}\multirow{3}{*}{soc-Slashdot0902} & 1.00 & 0.68 & 0.62 & 0.98 & 1.00 & 0.87 & 0.69 & 0.46 & 0.84 & 0.91 & 2.67  \\
                                  & 3.20 & 0.61 & 2.82 & 0.99 & 1.00 & 2.95 & 0.77 & 3.80 & 0.86 & 1.00 & 0.82  \\
                                  & 0.31 & 1.13 & 0.22 & 0.98 & 1.00 & 0.30 & 0.89 & 0.12 & 0.98 & 0.91 &      \\
\cmidrule(r){2-12} 
\multicolumn{1}{r}{H} & 0.33 & 0.10 & 0.12 & 0.30 & 0.42 & 0.33 & 0.09 & 0.14 & 0.19 & 0.31 & 5.26\\
\multicolumn{1}{r}{G}   & 0.55 & 0.10 & 0.24 & 0.33 & 0.44 & 0.53 & 0.09 & 0.31 & 0.22 & 0.34  & 3.03\\
\multicolumn{1}{r}{H/G} & 0.59 & 0.94 & 0.50 & 0.92 & 0.95 & 0.62 & 0.94 & 0.42 & 0.88 & 0.94\\
\cmidrule(r){2-12} 
\end{tabular}
\end{table*}



